Large Language Models as 'Hidden Persuaders': Fake Product Reviews are Indistinguishable to Humans and Machines

Reading and evaluating product reviews is central to how most people decide what to buy and consume online. However, the recent emergence of Large Language Models and Generative Artificial Intelligence now means writing fraudulent or fake reviews is potentially easier than ever. Through three studies we demonstrate that (1) humans are no longer able to distinguish between real and fake product reviews generated by machines, averaging only 50.8% accuracy overall - essentially the same that would be expected by chance alone; (2) that LLMs are likewise unable to distinguish between fake and real reviews and perform equivalently bad or even worse than humans; and (3) that humans and LLMs pursue different strategies for evaluating authenticity which lead to equivalently bad accuracy, but different precision, recall and F1 scores - indicating they perform worse at different aspects of judgment. The results reveal that review systems everywhere are now susceptible to mechanised fraud if they do not depend on trustworthy purchase verification to guarantee the authenticity of reviewers. Furthermore, the results provide insight into the consumer psychology of how humans judge authenticity, demonstrating there is an inherent 'scepticism bias' towards positive reviews and a special vulnerability to misjudge the authenticity of fake negative reviews. Additionally, results provide a first insight into the 'machine psychology' of judging fake reviews, revealing that the strategies LLMs take to evaluate authenticity radically differ from humans, in ways that are equally wrong in terms of accuracy, but different in their misjudgments.

==> exp/4-results.tex <==
\subsection{Results}
The main aim of the analysis: (1) measure human performance; (2) provide insights into the why behind the decisions: demographics (age, gender, education, language), AI knowledge, patterns of the provided product reviews (linguistic, stylistic, tone, emotional depth etc), confidence -- participants' implicit understanding.

The key research questions that guide the analysis are as follows:
\begin{enumerate}
    \item How well can participants distinguish AI-generated (fake) vs. human-written (real) reviews?
    \item Does participant demographics group or LLM experience impact performance?
    \item What factors make reviews harder to distinguish?
    \item Can LLMs do a better job than human?
\end{enumerate}

%Do AI-generated reviews that appear “too human-like” cause hesitation? Do very short or very long reviews create cognitive overload? Are specific words or phrases linked to slower classifications? Additionally, it is worth investigating whether low-confidence decisions tend to take longer, indicating uncertainty-driven delays. 

%To ensure the reliability of the follow-up analysis, we retained responses from participants who spent a reasonable amount of time on reviews, as these reflect deliberate decision-making. However, responses completed in under five minutes may lack meaningful engagement, making them uninformative or rushed guesses. As a result, these outliers were removed to maintain data quality and validity.

\subsubsection{RQ1}

\subsubsection{RQ2}

\subsubsection{RQ3}

\subsubsection{RQ4}



==> exp/Exp1-old-version.tex <==
Study A: LLM’s understanding capability

•Test how well LLMs understand customer reviews through classification tasks.

•Compare performance against domain experts, novices and classification models.

% a-Introduction of the experiment

% b-Experiment setting
%b-1-Data

%b-2-Ground truth collection

%b-3-LLM settings

% c-Experiment results
%c-1-LLM stability, domain experts' consistency
% TODO-evaluate results of two domain experts
% TODO-experiment with the most advanced models (open sourced and closed sourced)

%c-2-LLMs vs. ground truth vs. baselines
% TODO-extend experiments with other baselines


==> exp/Exp1.tex <==
%an exploration on the performance; implications to experiment design

\subsection{Initial observations}
In a pilot study, we explored the use of relatively basic prompts with Open AI models to generate fake reviews. However, the content produced by the LLM tends to be quite structured and consistent, e.g., following fixed patterns in sentence structure, length, and style. In contrast, human-written reviews generally do not adhere to such rigid patterns and typically exhibit the following characteristics:
\begin{itemize}
    \item Unstructured and inconsistent: Human reviews often contain spelling mistakes, grammatical errors, and incomplete sentences. In contrast, LLMs are trained on large datasets to produce "perfect" language patterns, which means they are less likely to replicate such imperfections.
    \item Diversity in style and expression: Human reviews reflect the unique language styles, emotional tones, and personal habits of different users. However, LLMs tend to learn from data that represents clear and relatively consistent patterns, limiting their ability to replicate this diversity.
    \item Ambiguity: Human reviews often express subjective opinions and emotions, which can sometimes be ambiguous. LLMs, on the other hand, typically generate content that is more neutral and structured, even when attempting to simulate emotional expression.
    \item Noise and irrelevance: Human reviews often contain irrelevant information, repetition, or rhetorical complaints. If LLMs attempt to mimic this level of "noise," the output might appear chaotic. Conversely, if the language is overly polished and structured, it can feel unnatural.
\end{itemize}

Overall, the analysis on the initial set of fake reviews suggest that LLMs face limitations in this type of task without task-specific training. LLMs are designed to produce linguistically "correct" text rather than imitate the inconsistent, imperfect nature of human expression. 

\subsection{Fake review generation}
To further explore this area, there are two potential directions for improving LLM performance on this task:
\begin{itemize}
    \item Fine-tuning: Training the pre-trained LLM on real noisy user-generated reviews could help it capture the spelling errors, grammatical mistakes, and emotional diversity found in human reviews.
    \item Prompt engineering: By designing prompts that include human heuristics for generating reviews, we might guide the model to produce content that appears more "human-like".
\end{itemize}

The objective of this study is not to verify better methods for generating fake reviews but to investigate whether humans can distinguish between real and fake reviews. Therefore, we opted for a more cost-effective approach focused on prompt engineering.

A set of fake reviews was generated using a carefully designed prompt, as detailed in Appendix A. The prompt incorporates specific heuristics and restricts the context to the product information that the reviews are intended to reference. 

\subsection{Experiment setting}
The review dataset includes 100 reviews, 46\% are labelled as “Real” while 54\% are labelled as “Machine Generated”. This is a moderately balanced dataset, leaning slightly toward machine-generated reviews.

13 machine learning experts participated in this experiment. They were provided with the same set of reviews to label. 

\subsection{Results}
[To-add: a confusion matrix]

The average accuracy achieved was 57.69\%, which is slightly better than random guessing but leaves significant room for improvement. 

Participants achieved an F1-score of 55.57\% for predicting real reviews. Their performance was slightly better for predicting machine-generated reviews, with an F1-score of 59.62\%, though there is still significant room for improvement.

This pilot study provided initial insights into the performance of LLMs in generating fake reviews and the challenges faced by machine learning experts in distinguishing them from real reviews. In subsequent experiments, we aim to collect more detailed participant data, conduct deeper analyses of the interactions between review text features and human performance and explore the performance of a wider range of participants. This will allow us to derive more actionable insights into the challenges of distinguishing real from fake reviews.

==> exp/Exp2.tex <==

\input{exp/1-analyse-reviews}

\input{exp/2-generate-reviews}

\input{exp/3-experiment-setting}

\input{exp/4-results}





==> exp/table-prompt-pilot.tex <==
% prompt version - used for N/Lab exp
\begin{table}[h]
\centering
\caption{Proposed prompts and corresponding design insights. - used in the pilot exp.}
\begin{tabular}{p{11.5cm}|p{3.5cm}}
    \hline\hline
    \textbf{Prompt} & \textbf{Justification and related insights} \\
    \hline
    Consider the following table: [table content] & Input context (source data)\\\hline
    For the above table, Please append three new columns: 1) rating (a numeric rating between 1and 5) 2) title (a short review title) 3) text (a review text). The new columns should contain product reviews as similar to human-written as possible. Generate the review based on the available row information. For each product row, provide exactly one new review. Format the final output as a table with the original columns plus the new ones appended at the end. & Expected output and formatting requirements\\\hline
    You should ensure that the reviews are as similar as possible to human writing’s typos, emotion, sentiment, punctuation style, etc. & 2, 6, 7 \\
    \hline
    Include a variety of reviews across the full rating scale, from low to high. & 7 \\
    \hline
    Please ensure you vary the number of sentences within the review (ensure some have 1 sentence maximum, some have two, some have three, and some have four) and also ensure you vary sentence length - some sentences can have only one or two words maximum even, if persuasive. & 1 \\
    \hline
    Ensure that there are an average number of 5 typographic or spelling mistakes for every 10 reviews generated. & 6 \\
    \hline
    Please vary the punctuation style (but do not use semicolons). & 2 \\
    \hline
    Please use slang, idiom, or metaphor if it is similar to normal reviews that might be created for the respective products. & 5 \\
    \hline
    Episodic memory or nostalgia can be used to give a sense that the product was actually used, or perhaps if the product is broken, is not delivered properly, or does not work as expected. & 4, 7 \\
    \hline
    The aim should be that a reader cannot distinguish the reviews from standard writing that might be expected on a website such as Amazon.com. & Main objective \\
    \hline\hline
\end{tabular}
\label{tab:prompt-pilot}
\end{table}


==> figs/tables.tex <==
% cm-both
\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[height=6cm,width=7cm]{figs/confusion_matrix_human.png}
    \caption{Confusion matrix - human}
    \label{cm-human}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[height=6cm,width=7cm]{figs/confusion_matrix_llms.png}
    \caption{Confusion matrix - LLMs}
    \label{cm-llm}
\end{subfigure}
\caption{Comparison of confusion matrices: human vs LLMs}
\label{fig:cm-comparison}
\end{figure}

% cm-human
\begin{figure}[htbp]
\centering
\includegraphics[height=6cm,width=7cm]{figs/confusion_matrix_human.png}
\label{cm-human}
\caption{Confusion matrix - human}
\end{figure}

% cm-llm
\begin{figure}[htbp]
\centering
\includegraphics[height=6cm,width=7cm]{figs/confusion_matrix_llms.png}
\label{cm-llm}
\caption{Confusion matrix - llms}
\end{figure}

% age vs accuracy
\begin{figure}[htbp]
\centering
\includegraphics[height=6cm,width=8cm]{figs/human accuracy age curve.png}
\label{human-age-accuracy}
\caption{Participant Age vs Accuracy}
\end{figure}

% accuracy in fake vs. real
\begin{figure}[htbp]
\centering
\includegraphics[height=6cm,width=6cm]{figs/human accuracy real vs fake.png}
\label{human-accuracy-real-fake}
\caption{Participant Accuracy in Fake vs Real reviews}
\end{figure}

% accuracy curve
\begin{figure}[htbp]
\centering
\includegraphics[height=6cm,width=8cm]{figs/human review accuracy curve.png}
\label{human-age-accuracy}
\caption{Participant AVG accuracy across trials}
\end{figure}

% confidence curve
\begin{figure}[htbp]
\centering
\includegraphics[height=6cm,width=8cm]{figs/human review confidence curve.png}
\label{human-confidence-accuracy}
\caption{Participant AVG confidence across trials}
\end{figure}

% duration curve
\begin{figure}[htbp]
\centering
\includegraphics[height=6cm,width=8cm]{figs/human review duration curve.png}
\label{human-duration-accuracy}
\caption{Participant AVG review duration (time spent) across trials}
\end{figure}

% feature correlation - both
\begin{figure}[htbp]
\centering
\includegraphics[height=4cm,width=16cm]{figs/review_features_correlation_real_vs_fake.png}
\label{feature-correlation-both}
\caption{Feature correlation}
\end{figure}

% feature correlation - real
\begin{figure}[htbp]
\centering
\includegraphics[height=4cm,width=9cm]{figs/review features correlations with performance.png}
\label{feature-correlation-real}
\caption{Feature correlation - real reviews}
\end{figure}

% feature correlation - fake
\begin{figure}[htbp]
\centering
\includegraphics[height=4cm,width=9cm]{figs/review features correlations with performance-fake.png}
\label{feature-correlation-fake}
\caption{Feature correlation - fake reviews}
\end{figure}

